Arkade: k-Nearest Neighbor Search With Non-Euclidean Distances using GPU Ray Tracing

High-performance implementations of $k$-Nearest Neighbor Search ($k$NN) in low dimensions use tree-based data structures. Tree algorithms are hard to parallelize on GPUs due to their irregularity. However, newer Nvidia GPUs offer hardware support for tree operations through ray-tracing cores. Recent works have proposed using RT cores to implement $k$NN search, but they all have a hardware-imposed constraint on the distance metric used in the search -- the Euclidean distance. We propose and implement two reductions to support $k$NN for a broad range of distances other than the Euclidean distance: Arkade Filter-Refine and Arkade Monotone Transformation, each of which allows non-Euclidean distance-based nearest neighbor queries to be performed in terms of the Euclidean distance. With our reductions, we observe that $k$NN search time speedups range between $1.6$x-$200$x and $1.3$x-$33.1$x over various state-of-the-art GPU shader core and RT core baselines, respectively. In evaluation, we provide several insights on RT architectures' ability to efficiently build and traverse the tree by analyzing the $k$NN search time trends.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

main.pdf:  main.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done





